On the Reduction of Variance and Overestimation of Deep Q-Learning

The breakthrough of deep Q-Learning on different types of environments revolutionized the algorithmic design of Reinforcement Learning to introduce more stable and robust algorithms, to that end many extensions to deep Q-Learning algorithm have been proposed to reduce the variance of the target values and the overestimation phenomena. In this paper, we examine new methodology to solve these issues, we propose using Dropout techniques on deep Q-Learning algorithm as a way to reduce variance and overestimation. We also present experiments conducted on benchmark environments, demonstrating the effectiveness of our methodology in enhancing stability and reducing both variance and overestimation in model performance.

==> Experiments.tex <==
\section{Experiments}
\paragraph The experiments were designed to address the following questions:
\begin{itemize}
\item How does Dropout affect the variance in DQN and the overestimation error.
\item How How does Dropout affect the learned polices
quality.
\end{itemize}
To that end, we ran Dropout DQN and DQN on one of classic control environments. Additionally, we ran Dropout DQN and DQN on a Gridworld toy problem where the optimal value function can be computed exactly.
\subsection{Classic Control Environment}
To evaluate Dropout DQN, we adopt the typical RL
methodology where agent performance is measured at the
end of training. Thus we ran ten consecutive learning trails and average them. We have evaluated Dropout DQN algorithm on Cartpole from the Classic Control Environment. The game of Cartpole was selected due to its popularity and the relative ease of the DQN to reach a steady state policy.
As can be seen in Figure 3 and Tabel
\ for all ten learning trails, using DQN with different Dropout methods results in better-preforming policies, and less variability between the
runs of independent learning trials.
Overall, the results suggest that in practice Dropout can be
used to reduces variance and overestimation, which leads to
stabilized learning curves and significantly improved
performance.
\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics[width=.5\textwidth] {A.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.
